Your Next State-of-the-Art Could Come from Another Domain: A Cross-Domain Analysis of Hierarchical Text Classification

Text classification with hierarchical labels is a prevalent and challenging task in natural language processing. Examples include assigning ICD codes to patient records, tagging patents into IPC classes, assigning EUROVOC descriptors to European legal texts, and more. Despite its widespread applications, a comprehensive understanding of state-of-the-art methods across different domains has been lacking. In this paper, we provide the first comprehensive cross-domain overview with empirical analysis of state-of-the-art methods. We propose a unified framework that positions each method within a common structure to facilitate research. Our empirical analysis yields key insights and guidelines, confirming the necessity of learning across different research areas to design effective methods. Notably, under our unified evaluation pipeline, we achieved new state-of-the-art results by applying techniques beyond their original domains.

==> app.tex <==

\section{Details of the submodules used in recent methods}\label{sec:details-submodules}

Table~\ref{tab:submodules} shows the submodules used in recent methods.

\begin{sidewaystable}[!h]
    \tiny
    \centering
    \caption{Submodules used in recent methods}
    \label{tab:submodules}
    \begin{tabular}{cccccccc}
    \toprule
    Method & Text Encoder & Label Encoder & Out space seg & Text-Label info fusion & Training objectives & Score Prediction & Prediction Refinement \\ 
    \midrule
    XR-Transformer & LLM\footnotemark[0]\&TF-IDF & PIFA & PLT & - & \makecell{(Multi-stage) CLS loss\footnotemark[1]+ \\Contrastive (MAN+TFN)} & MS Linear & MS ranker \\ 
    MatchXML & LLM\footnotemark[0]\&TF-IDF & Label2Vec & PLT & Embedding alignment & \makecell{(Multi-stage) CLS loss + \\ Contrastive (MAN+TFN) \\+ Alignment loss} & MS Linear &  MS ranker \\ 
    HILL & LLM\footnotemark[0] & Coding Tree & - & Structure encoder\footnotemark[2] & \makecell{CLS loss + \\NT-Xent contrastive loss}& Linear & -\\ 
    HiAGM-TP & GRU + CNN & Tree-LSTM/GCN & - & Structure encoder\footnotemark[3] & CLS loss with regularization& Linear& -\\ 
    HiAGM-LA & GRU + CNN & Tree-LSTM/GCN & - & Structured label attn & CLS loss with regularization& Linear& -\\ 
    PLM-ICD & LLM\footnotemark[0] & -& -& \makecell{Segmented text\\ with label-aware attn}& CLS loss & Linear & - \\ 
    FlatBERT\footnotemark[4] & LLM\footnotemark[0] & - & - & - & CLS loss & Linear & -\\ 
    THMM & LLM\footnotemark[0] & - & Original taxonomy & \makecell{Parent-kid \\representation concatenation} & CLS loss & An MLP per class & - \\ 
    HR-SciBERT-mt & LLM\footnotemark[0] & - & Original taxonomy & \makecell{Parent-kid \\parameter sharing} & \makecell{CLS loss + \\Keyword prediction loss}  & An MLP per class & - \\ 
    X-Transformer & LLM \& TF-IDF &  PIFA  & PLT & - &  \makecell{CLS loss + \\Contrastive (MAN+TFN)} & Linear & 1-stage ranker \\ 
    XR-Linear & TF-IDF & PIFA & PLT & - &  \makecell{MS CLS loss + \\Contrastive (MAN+TFN)} & MS Linear & MS ranker  \\ 
    AttentionXML & LSTM & PIFA & PLT & label attn & (Multi-Stage) CLS & MS Linear & -  \\ 
    Bonsai & TF-IDF & PIFA & PLT  & - & (Multi-Stage) CLS & MS Linear &  - \\ 
    HVHMC & GCN (word-doc)  & \makecell{GCN(label-word) \\ inter+intra level dependency} & - & repr concat & \makecell{local + \\global CLS} & \makecell{level-wise +\\all cat} & - \\ 
    HGCLR & LLM & Graphnomer & - & \makecell{label guided \\ positive sample gen} & \makecell{CLS +\\ NT-Xent contrastive} & Linear & - \\ 
    HBGL & LLM & LLM with custom pretraining task & - & \makecell{Repr concat +\\ custom attn mask} & \makecell{Multi-stage CLS +\\ label mask pretraining} & level-wise & - \\ 
    HARNN & LSTM & dense vec & - & HAM &  \makecell{local + \\global CLS} & \makecell{level-wise +\\all cat} & -  \\ 
    HTrans & \makecell{GRU +\\modified outputs} & - & Original taxonomy & \makecell{Parent-kid \\parameter sharing} & CLS &  An MLP per class & -  \\ 
    PARL & \makecell{LLM (bi+cross) +\\GraphSAGE+\\BM25} & LLM & - & Bi-enc + Cross-enc & Ranknet loss &  L2R & - \\  
    HyperIM & Hyperbolic & Hyperbolic & - & \makecell{Label-aware\\doc repr\\(geodesic distance)} & \makecell{CLS loss + \\Contrastive} & emb sim & - \\ 
    LA-HCN & LSTM & dense vec & - & \makecell{Level-wise label attn+\\label-component assoc.} & \makecell{local + \\global CLS} & \makecell{combine\\local+global} & - \\ 
    HCSM & CNN+LSTM & w2v  & - & \makecell{HARNN+\\HON-LSTM+\\HBiCaps} & Margin loss & 1 cap for 1 class & - \\ 
    HiLAP & CNN & dense vec & Original taxonomy & - & \makecell{Neg discounted\\cum rewards} & Policy network & - \\ 
    ExMLDS & \makecell{TF-IDF+\\ADMM projection} & \makecell{skip-gram +\\SPPMI factorization} & - & ADMM projection & \makecell{CLS +\\skig-gram neg+\\label co-occurance reg} & emb similarity & - \\ 
    GalaXC & Fixed pre-trained & \makecell{GNN +\\label attention} & ANNS & Joint doc-label graph  & \makecell{CLS loss + \\neg Contrastive} & emb sim & - \\ 
    EcLARE & TF-IDF & \makecell{GCN + \\label attention} & \makecell{Graph-Assisted\\Multi-label\\Expansion (GAME)}  & - & \makecell{CLS loss + \\neg Contrastive +\\spectral reg} & emb sim & - \\ 
    \midrule
    \multicolumn{8}{l}{\textbf{Plug-in Methods (can be combined with methods above):}} \\
    \multicolumn{8}{l}{\textit{Training Objective Enhancements:}} \\
    DepReg & \multicolumn{7}{l}{Adds dependency regularization term to training objectives} \\
    \multicolumn{8}{l}{\textit{Label Space Processing:}} \\
    PS-PLT & \multicolumn{7}{l}{Enhances PLT with propensity scoring for better label space segmentation} \\
    \multicolumn{8}{l}{\textit{Prediction Refinement:}} \\
    Capsule Net & \multicolumn{7}{l}{Replaces standard prediction with capsule network + label correlation restrictions} \\
    CorNet & \multicolumn{7}{l}{Adds correlation-based prediction refinement layer} \\
    \multicolumn{8}{l}{\textit{Data Augmentation:}} \\
    GANDALF & \multicolumn{7}{l}{Graph-based data augmentation for long-tail labels} \\
    REMIDIAL & \multicolumn{7}{l}{Data augmentation through label correlation patterns} \\
    \botrule
    \end{tabular}
        \footnotetext[0]{LLM: Large Language Model, e.g. BERT, RoBERTa, etc. Specifically, we use BERT as the default LLM encoder except for the following cases: RoBERTa-PM for PLM-ICD on MIMIC3-3681 and SciBERT for THMM on USPTO2M-632 following the original papers.}
        \footnotetext[1]{Classification loss for multi-label classification, depending on the specific loss function used, most commonly the binary cross-entropy loss.}
        \footnotetext[2]{A custom defined structure encoder that propagates information from the leaf nodes to the root node of the coding tree.}
        \footnotetext[3]{Tree-LSTM or GCN, corresponding to the label encoder.}
        \footnotetext[4]{PatentBERT in the original paper due to its application in patent classification. We rename it as FlatBERT for generalization.}
\end{sidewaystable}



\section{Additional experiment results}\label{sec:additional-results}
\subsection{Impact of Different k Values}\label{sec:k-value-analysis}
While the main text focuses on Precision/Recall@1, analyzing model behaviors at k=3, 5, 8, 10 reveals additional insights into multi-label prediction capabilities (Tables~\ref{tab:cross-domain-precision-scores-ranks-3}, \ref{tab:cross-domain-recall-scores-ranks-3}, \ref{tab:cross-domain-precision-scores-ranks-5}, \ref{tab:cross-domain-recall-scores-ranks-5}, \ref{tab:cross-domain-precision-scores-ranks-8}, \ref{tab:cross-domain-recall-scores-ranks-8}, \ref{tab:cross-domain-precision-scores-ranks-10}, \ref{tab:cross-domain-recall-scores-ranks-10})

\paragraph{Precision-Recall Trade-offs} All datasets show precision decreases and recall increases as $k$ grows, but with notably different magnitudes. WOS shows dramatic precision drops ($\sim$70 percentage points from $k=1$ to $k=10$, e.g., HILL: 90.81$\rightarrow$19.31) due to its having only two labels per document. MIMIC3 exhibits more gradual degradation ($\sim$25 points, e.g., PLM-ICD: 90.77$\rightarrow$67.11) for its high label cardinality. EurLex-3985 demonstrates the most stable precision metrics with only $\sim$6-7 point drops from $k=1$ to $k=5$ (XR-Transformer: 97.67$\rightarrow$90.91).

\paragraph{Model Ranking Changes}
Analysis of model rankings across $k=1,3,5,8,10$ reveals several consistent patterns and notable shifts. Some models maintain stable leadership positions: XR-Transformer consistently ranks first on NYT-166 and EurLex-3985, HILL maintains first place on WOS-141, and PLM-ICD leads on MIMIC3-3681 across all $k$ values. However, significant ranking changes emerge on certain datasets. PLM-ICD shows marked improvement on SciHTC-83, climbing from rank 4 (k=1) to rank 1 (k=8,10), while HILL demonstrates similar improvement on EurLexDC-410, advancing from rank 4 to rank 1. Conversely, some models experience performance degradation at higher k values: MatchXML drops from rank 1 to rank 5 on SciHTC-83, and XR-Transformer declines from rank 3 to rank 7 on the same dataset. The most stable rankings across k values are observed for XR-Transformer on NYT-166, EurLex-3985, and USPTO2M-632, HILL on WOS-141, and PLM-ICD on MIMIC3-3681. 


\begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Precision@3 Scores and Ranks}
    \label{tab:cross-domain-precision-scores-ranks-3}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 57.28 - 5 & 84.67 - 2 & 94.36 - 2 & 38.92 - 2 & 39.90 - 1 & 25.79 - 1 & 79.42 - 3 & 44.22 - 3 \\
    XR-Transformer & 57.65 - 4 & 85.16 - 1 & 94.67 - 1 & 39.02 - 1 & 39.35 - 5 & 25.15 - 2 & 80.04 - 2 & 42.75 - 4 \\
    HILL & 60.23 - 1 & 81.83 - 4 & 92.27 - 3 & 37.94 - 3 & 36.56 - 8 & 21.84 - 7 & 71.31 - 4 & \texttt{ET} \\
    HiAGM-TP & 60.10 - 2 & 73.76 - 7 & 87.19 - 5 & 37.19 - 5 & 36.93 - 7 & 23.35 - 6 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 59.17 - 3 & 84.04 - 3 & 91.37 - 4 & 37.81 - 4 & 39.65 - 3 & 24.04 - 4 & 85.64 - 1 & 44.57 - 2 \\
    FlatBERT & 34.81 - 7 & 75.23 - 6 & 42.53 - 7 & 6.55 - 7 & 38.99 - 6 & 23.95 - 5 & 19.46 - 5 & 44.85 - 1 \\
    THMM & 57.24 - 6 & 81.74 - 5 & 54.32 - 6 & 22.17 - 6 & 39.83 - 2 & 24.63 - 3 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 39.44 - 4 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Recall@3 Scores and Ranks}
    \label{tab:cross-domain-recall-scores-ranks-3}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 85.93 - 5 & 53.97 - 2 & 23.36 - 2 & 93.28 - 2 & 66.70 - 1 & 50.30 - 1 & 19.22 - 3 & 78.23 - 3 \\
    XR-Transformer & 86.47 - 4 & 54.36 - 1 & 23.46 - 1 & 93.62 - 1 & 65.83 - 4 & 48.94 - 2 & 19.38 - 2 & 76.19 - 4 \\
    HILL & 90.34 - 1 & 51.33 - 5 & 22.79 - 3 & 91.62 - 3 & 60.98 - 8 & 42.26 - 7 & 17.01 - 4 & \texttt{ET} \\
    HiAGM-TP & 90.16 - 2 & 47.09 - 6 & 21.49 - 5 & 89.89 - 5 & 61.41 - 7 & 45.05 - 6 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 88.75 - 3 & 53.45 - 3 & 22.60 - 4 & 90.96 - 4 & 66.34 - 3 & 46.44 - 5 & 20.94 - 1 & 78.70 - 2 \\
    FlatBERT & 52.22 - 7 & 46.08 - 7 & 9.87 - 7 & 18.40 - 7 & 65.41 - 6 & 47.27 - 4 & 4.15 - 5 & 79.04 - 1 \\
    THMM & 85.86 - 6 & 51.42 - 4 & 12.82 - 6 & 56.37 - 6 & 66.54 - 2 & 47.59 - 3 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 65.78 - 5 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Precision@5 Scores and Ranks}
    \label{tab:cross-domain-precision-scores-ranks-5}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 36.29 - 5 & 72.24 - 2 & 90.69 - 2 & 23.87 - 2 & 27.73 - 4 & 18.52 - 1 & 72.77 - 3 & 29.75 - 3 \\
    XR-Transformer & 36.67 - 4 & 72.58 - 1 & 90.91 - 1 & 24.01 - 1 & 27.30 - 6 & 17.93 - 3 & 73.32 - 2 & 28.60 - 4 \\
    HILL & 37.53 - 1 & 69.69 - 5 & 88.94 - 3 & 23.70 - 3 & 25.75 - 8 & 15.97 - 7 & 64.29 - 4 & \texttt{ET} \\
    HiAGM-TP & 37.39 - 2 & 61.81 - 7 & 82.97 - 5 & 23.22 - 5 & 26.47 - 7 & 17.11 - 6 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 37.10 - 3 & 71.89 - 3 & 87.11 - 4 & 23.40 - 4 & 27.97 - 2 & 17.80 - 4 & 80.02 - 1 & 30.46 - 2 \\
    FlatBERT & 23.77 - 7 & 64.12 - 6 & 37.70 - 7 & 4.15 - 7 & 27.56 - 5 & 17.52 - 5 & 14.38 - 5 & 30.71 - 1 \\
    THMM & 35.73 - 6 & 69.73 - 4 & 47.55 - 6 & 14.79 - 6 & 28.05 - 1 & 18.05 - 2 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 27.95 - 3 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Recall@5 Scores and Ranks}
    \label{tab:cross-domain-recall-scores-ranks-5}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 90.72 - 5 & 66.57 - 2 & 37.20 - 2 & 94.74 - 2 & 76.71 - 4 & 59.79 - 1 & 28.58 - 3 & 84.44 - 3 \\
    XR-Transformer & 91.67 - 4 & 66.88 - 1 & 37.31 - 1 & 95.31 - 1 & 75.53 - 6 & 57.67 - 3 & 28.80 - 2 & 81.97 - 4 \\
    HILL & 93.83 - 1 & 63.00 - 5 & 36.39 - 3 & 94.20 - 3 & 71.33 - 8 & 51.54 - 7 & 24.94 - 4 & \texttt{ET} \\
    HiAGM-TP & 93.48 - 2 & 57.34 - 6 & 33.81 - 5 & 92.76 - 5 & 73.01 - 7 & 55.22 - 6 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 92.75 - 3 & 66.04 - 3 & 35.67 - 4 & 93.08 - 4 & 77.41 - 2 & 57.43 - 4 & 31.67 - 1 & 85.93 - 2 \\
    FlatBERT & 59.41 - 7 & 56.46 - 7 & 14.53 - 7 & 18.99 - 7 & 76.40 - 5 & 57.35 - 5 & 5.19 - 5 & 86.40 - 1 \\
    THMM & 89.33 - 6 & 63.77 - 4 & 18.61 - 6 & 61.25 - 6 & 77.58 - 1 & 58.17 - 2 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 77.21 - 3 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Precision@8 Scores and Ranks}
    \label{tab:cross-domain-precision-scores-ranks-8}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 23.36 - 5 & 60.60 - 2 & 83.40 - 2 & 15.07 - 3 & 19.03 - 5 & 13.10 - 1 & 63.90 - 3 & 19.83 - 3 \\
    XR-Transformer & 23.56 - 4 & 61.04 - 1 & 83.55 - 1 & 15.16 - 2 & 18.67 - 6 & 12.63 - 4 & 64.22 - 2 & 19.02 - 4 \\
    HILL & 23.96 - 1 & 58.32 - 4 & 82.18 - 3 & 15.19 - 1 & 17.91 - 8 & 11.56 - 7 & 55.18 - 4 & \texttt{ET} \\
    HiAGM-TP & 23.82 - 2 & 50.89 - 7 & 75.94 - 5 & 14.84 - 5 & 18.64 - 7 & 12.43 - 6 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 23.74 - 3 & 60.53 - 3 & 79.29 - 4 & 14.90 - 4 & 19.52 - 1 & 12.95 - 3 & 72.07 - 1 & 20.60 - 2 \\
    FlatBERT & 16.84 - 7 & 54.00 - 6 & 31.73 - 7 & 2.63 - 7 & 19.19 - 4 & 12.61 - 5 & 8.99 - 5 & 20.79 - 1 \\
    THMM & 23.02 - 6 & 58.14 - 5 & 39.24 - 6 & 10.21 - 6 & 19.43 - 3 & 13.04 - 2 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 19.50 - 2 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Recall@8 Scores and Ranks}
    \label{tab:cross-domain-recall-scores-ranks-8}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 93.42 - 5 & 78.53 - 2 & 54.08 - 2 & 95.50 - 3 & 83.87 - 5 & 67.32 - 1 & 38.82 - 3 & 88.08 - 3 \\
    XR-Transformer & 94.24 - 4 & 79.02 - 1 & 54.18 - 1 & 96.09 - 2 & 82.29 - 6 & 64.73 - 5 & 39.01 - 2 & 85.43 - 4 \\
    HILL & 95.83 - 1 & 74.47 - 5 & 53.21 - 3 & 96.13 - 1 & 79.13 - 8 & 59.69 - 7 & 33.24 - 4 & \texttt{ET} \\
    HiAGM-TP & 95.27 - 2 & 67.05 - 7 & 48.92 - 5 & 94.46 - 5 & 82.03 - 7 & 64.26 - 6 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 94.97 - 3 & 78.18 - 3 & 51.30 - 4 & 94.47 - 4 & 86.11 - 1 & 66.85 - 3 & 44.03 - 1 & 90.54 - 2 \\
    FlatBERT & 67.38 - 7 & 68.51 - 6 & 19.65 - 7 & 19.14 - 7 & 84.71 - 4 & 65.83 - 4 & 5.19 - 5 & 91.03 - 1 \\
    THMM & 92.09 - 6 & 75.55 - 4 & 24.37 - 6 & 66.87 - 6 & 85.68 - 3 & 67.07 - 2 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 85.92 - 2 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Precision@10 Scores and Ranks}
    \label{tab:cross-domain-precision-scores-ranks-10}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 18.86 - 5 & 54.61 - 2 & 78.01 - 2 & 12.10 - 3 & 15.75 - 5 & 10.98 - 3 & 58.77 - 3 & 16.21 - 3 \\
    XR-Transformer & 19.01 - 4 & 55.01 - 1 & 78.14 - 1 & 12.17 - 2 & 15.43 - 7 & 10.58 - 5 & 58.92 - 2 & 15.55 - 4 \\
    HILL & 19.31 - 1 & 52.40 - 4 & 77.13 - 3 & 12.25 - 1 & 14.89 - 8 & 9.84 - 7 & 50.25 - 4 & \texttt{ET} \\
    HiAGM-TP & 19.20 - 2 & 45.79 - 7 & 70.91 - 5 & 11.98 - 5 & 15.60 - 6 & 10.58 - 5 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 19.17 - 3 & 54.55 - 3 & 73.61 - 4 & 12.01 - 4 & 16.21 - 1 & 10.99 - 2 & 67.11 - 1 & 16.94 - 2 \\
    FlatBERT & 14.54 - 7 & 48.22 - 6 & 28.70 - 7 & 2.20 - 7 & 15.95 - 4 & 10.71 - 4 & 7.19 - 5 & 17.08 - 1 \\
    THMM & 18.63 - 6 & 52.08 - 5 & 35.56 - 6 & 8.52 - 6 & 16.14 - 2 & 11.06 - 1 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 16.14 - 2 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    
    
    
    \begin{table}[!h]
    \footnotesize
    \centering
    \caption{Cross-Domain Recall@10 Scores and Ranks}
    \label{tab:cross-domain-recall-scores-ranks-10}
    \begin{tabular}{l@{\hskip 0.15in}cccccccc}
    \toprule
    \textbf{Method} & \makecell{\textbf{WOS} \\-141} & \makecell{\textbf{NYT} \\-166} & \makecell{\textbf{EurLex} \\-3985} & \makecell{\textbf{EurLexDC} \\-410} & \makecell{\textbf{SciHTC} \\-83} & \makecell{\textbf{SciHTC} \\-800} & \makecell{\textbf{MIMIC3} \\-3681} & \makecell{\textbf{USPTO2M} \\-632} \\
    \midrule
    MatchXML & 94.29 - 5 & 83.87 - 2 & 62.67 - 2 & 95.74 - 3 & 86.62 - 5 & 70.39 - 3 & 43.90 - 3 & 89.34 - 3 \\
    XR-Transformer & 95.05 - 4 & 84.38 - 1 & 62.79 - 1 & 96.34 - 2 & 84.91 - 7 & 67.64 - 6 & 43.99 - 2 & 86.68 - 4 \\
    HILL & 96.53 - 1 & 79.70 - 5 & 61.91 - 3 & 96.72 - 1 & 82.17 - 8 & 63.50 - 7 & 37.26 - 4 & \texttt{ET} \\
    HiAGM-TP & 96.01 - 2 & 71.85 - 7 & 56.67 - 5 & 95.10 - 4 & 85.78 - 6 & 68.27 - 5 & \texttt{ET} & \texttt{ET} \\
    PLM-ICD & 95.84 - 3 & 83.58 - 3 & 59.03 - 4 & 95.07 - 5 & 89.23 - 1 & 70.82 - 2 & 50.25 - 1 & 92.13 - 2 \\
    FlatBERT & 72.70 - 7 & 72.93 - 6 & 22.13 - 7 & 19.99 - 7 & 87.89 - 4 & 69.73 - 4 & 5.19 - 5 & 92.61 - 1 \\
    THMM & 93.13 - 6 & 80.65 - 4 & 27.56 - 6 & 69.44 - 6 & 88.81 - 3 & 70.99 - 1 & \texttt{ET} & \texttt{ET} \\
    HR-SciBERT-mt & \texttt{ET} & \texttt{ET} & \texttt{ET} & \texttt{ET} & 88.83 - 2 & \texttt{ET} & \texttt{ET} & \texttt{ET} \\
    \botrule
    \end{tabular}
    \end{table}
    



\subsection{Dataset- and Method-Specific Patterns}\label{sec:dataset-method-specific-patterns}
\emph{Hierarchy depth} strongly influences the performance of certain methods. Shallow hierarchies (like in WOS-141) are better handled by HILL, HiAGM-TP, and THMM than datasets with deeper hierarchies (EurLex-*, SciHTC-*). \emph{Document length} and label structure are key factors because datasets with long documents and flat label structures (MIMIC3-3681, USPTO2M-632) seem to require specialized text processing approaches, which PLM-ICD handles effectively. Datasets with \emph{label sparsity}, i.e. with low average samples per label (EurLex-*), benefit from robust label-aware mechanisms, where MatchXML, XR-Transformer, and PLM-ICD excel. \emph{Sample abundance} can compensate for other complexities. For example, datasets with high sample counts per label (like SciHTC-83) enable even simpler methods to perform well, as demonstrated by THMM's unexpected success.

On the method side, the \emph{baseline} FlatBERT lags behind other methods but shows competitive results with sufficient training data (USPTO2M-632). \emph{Transformer-based} methods (MatchXML, XR-Transformer) excel with large label spaces but show limitations in exploiting label redundancy. 
\emph{Per node classification} methods face scalability issues, as HR-SciBERT-mt usually exceeds time limits.


\subsection{XR-Transformer Tree Initialization Variations}\label{sec:xr-tree-init}
The results (\ref{tab:xrt-precision-1}, \ref{tab:xrt-recall-1}) demonstrate that tree initialization methods have a small but consistent impact on XR-Transformer's performance. Random initialization consistently performs slightly worse than both PIFA and Gold methods across most datasets, with performance gaps of 0.1-0.5 percentage points in both precision and recall. Gold initialization generally achieves the best results (e.g., 97.67\% precision on EurLex-3985), followed closely by PIFA, while Random initialization ranks last. This suggests that leveraging either Gold or PIFA tree structures is beneficial, though the performance differences are modest.

\begin{table}[!htb]
    \tiny
    \centering
    \caption{XR-Transformer tree initialization variations precision@1}
    \label{tab:xrt-precision-1}
    \begin{tabular}{cccccccccc}
    \toprule
    Init Tree & WOS-141 & NYT-166 & EurLex-3956 & EurLex-3985  & EurLexDC & SciHTC-83 & SciHTC-800 & MIMIC3-3681 (512) & USPTO2M-632\\ \midrule
    PIFA & 86.49 & 96.64 & 87.83 & 97.51 & 89.80 & 61.53 & 40.69 & 88.32 & 80.99 \\ 
    Gold & 86.39 & 96.70 & 88.06 & 97.67 & 89.86 & 61.58 & 40.76 & 88.03 & 81.19\\ 
    Random &86.40 & 96.71  & 86.77 & 97.48 & 89.79 & 61.37 & 40.68 & 87.69 & 80.82 \\ 
    \botrule
    \end{tabular}
\end{table}

\begin{table}[!htb]
    \tiny
    \centering
    \caption{XR-Transformer tree initialization variations recall@1}
    \label{tab:xrt-recall-1}
    \begin{tabular}{cccccccccc}
    \toprule
    Init Tree & WOS-141 & NYT-166 & EurLex-3956 & EurLex-3985  & EurLexDC & SciHTC-83 & SciHTC-800 & MIMIC3-3681 (512) & USPTO2M-632 \\ \midrule
    PIFA & 43.25 & 22.93 & 17.82 & 8.09 & 78.91  & 36.29  & 27.43  & 7.37 & 54.75 \\
    Gold & 43.20 & 22.94 & 17.88 & 8.10 & 78.96 & 36.32 & 27.49  & 7.35 & 54.90 \\ 
    Random & 43.20 & 22.95 & 17.62 & 8.08 & 78.91 & 36.21 & 27.42 & 7.31 & 54.66 \\
    \botrule
    \end{tabular}
\end{table}

